SHREC 2011: robust feature detection and description benchmark

Feature-based approaches have recently become very popular in computer vision and image analysis applications, and are becoming a promising direction in shape retrieval. SHREC'11 robust feature detection and description benchmark simulates the feature detection and description stages of feature-based shape retrieval algorithms. The benchmark tests the performance of shape feature detectors and descriptors under a wide variety of transformations. The benchmark allows evaluating how algorithms cope with certain classes of transformations and strength of the transformations that can be dealt with. The present paper is a report of the SHREC'11 robust feature detection and description benchmark results.

==> desc/litman-desc.tex <==
\textbf{SI-HKS} (Litman {\em et al.} \cite{litman2010diffusion}, using Bronstein and Kokkinos \cite{iasonas}). 
%
The scale-invariant heat kernel signature (SI-HKS) was proposed by Bronstein and Kokkinos \cite{iasonas} as a generalization of the HKS descriptor \cite{sun09hks}, computed as the diagonal of the heat diffusion kernel and multiple scales. Scale invariance in this descriptor is achieved by using the Fourier transform magnitude applied w.r.t. the scale parameter. 
%
To use the SI-HKS as a region descriptor, first the SI-HKS is computed at each point of the detected region. Next, a localized ``bag of features'' is computed for that region using vector quantization in a fixed vocabulary of descriptors \cite{bronstein2009shape}. 
%
For exact details and settings, see \cite{litman2010diffusion}. 





==> desc/smeets-desc.tex <==
\textbf{meshSIFT descriptor} (Smeets {\em et al.} \cite{Maes2010}). 
As feature descriptor, meshSIFT describes the neighbourhood of every scale space extremum.
In order to have an orientation-invariant descriptor, each feature point location is assigned a canonical orientation (more details in \cite{Maes2010}).
% 
The meshSIFT algorithm then describes the neighbourhood of every scale space extremum in a feature vector consisting of concatenated histograms of shape indices and slant angles. Each of these histograms is calculated over a small circular region. In each region we calculate two histograms with 8 bins each: one containing the shape index and the other containing the slant angles. First, each entry for both histograms is Gaussian weighted with the geodesic distance to the feature location and Gaussian weighted with the geodesic distance to the center of the region. Next, every histogram is normalized and clipped, reducing the influence of large histogram values. In a final step all histograms are concatenated leading to a 144D feature vector.

==> results/inverseCT_table_matchingScore.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 100.00} & {\small 100.00} & {\small 95.83} & {\small 96.88} & {\small 95.00}\\
{\small\em Rasterization} & {\small 88.89} & {\small 90.87} & {\small 93.92} & {\small 70.44} & {\small 56.35}\\
{\small\em Sampling} & {\small 1.00} & {\small 0.94} & {\small 0.96} & {\small 0.72} & {\small 0.57}\\
{\small\em Holes} & {\small 81.82} & {\small 40.91} & {\small 27.27} & {\small 20.45} & {\small 16.36}\\
{\small\em Micro holes} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 93.75} & {\small 81.00}\\
{\small\em Scaling} & {\small 0.00} & {\small 50.00} & {\small 66.67} & {\small 75.00} & {\small 80.00}\\
{\small\em Affine} & {\small 63.64} & {\small 46.10} & {\small 43.56} & {\small 40.17} & {\small 38.80}\\
{\small\em Noise} & {\small 77.78} & {\small 84.72} & {\small 81.48} & {\small 83.84} & {\small 81.07}\\
{\small\em Shot Noise} & {\small 81.82} & {\small 82.58} & {\small 59.81} & {\small 59.86} & {\small 51.89}\\
{\small\em Partial} & {\small 66.67} & {\small 61.90} & {\small 53.77} & {\small 50.74} & {\small 44.60}\\
{\small\em View} & {\small 0.00} & {\small 20.83} & {\small 23.41} & {\small 31.20} & {\small 34.96}\\
\hline
{\small{\textbf{Average}}} & {\small 69.15} & {\small 70.15} & {\small 67.41} & {\small 63.11} & {\small 57.96}\\
\hline
\end{tabular}
\caption{\small Robustness of SI-HKS region description algorithm ($\%$ of nearest neighbors with overlap {\em overlap $\geq$ 70\%}) on stable regions detected using egde-weight $1/c(v_1,v_2)$. \label{}}
\end{table}

==> results/inverse_HKS_table_matchingScore.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00}\\
{\small\em Rasterization} & {\small 73.33} & {\small 77.58} & {\small 66.00} & {\small 49.50} & {\small 41.42}\\
{\small\em Sampling} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 75.00} & {\small 60.00}\\
{\small\em Holes} & {\small 100.00} & {\small 50.00} & {\small 33.33} & {\small 25.00} & {\small 21.46}\\
{\small\em Micro holes} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 96.15} & {\small 84.07}\\
{\small\em Scaling} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 87.50} & {\small 86.25}\\
{\small\em Affine} & {\small 80.00} & {\small 58.75} & {\small 48.26} & {\small 43.34} & {\small 42.36}\\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 88.89} & {\small 79.17} & {\small 72.56}\\
{\small\em Shot Noise} & {\small 100.00} & {\small 100.00} & {\small 83.33} & {\small 75.00} & {\small 65.00}\\
{\small\em Partial} & {\small 75.00} & {\small 72.50} & {\small 60.45} & {\small 51.59} & {\small 41.27}\\
{\small\em View} & {\small 0.00} & {\small 50.00} & {\small 54.76} & {\small 59.82} & {\small 50.71}\\
\hline
{\small{\textbf{Average}}} & {\small 84.39} & {\small 82.62} & {\small 75.91} & {\small 67.46} & {\small 60.46}\\
\hline
\end{tabular}
\caption{\small Robustness of SI-HKS region description algorithm ($\%$ of nearest neighbors with overlap {\em overlap $\geq$ 70\%}) on stable regions detected using egde-weight $1/h_t(v_1,v_2)$ .\label{}}
\end{table}

==> results/keller_spin-1.feat.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 97.93} & {\small 98.50} & {\small 98.74} & {\small 98.77} & {\small 98.78} \\
{\small\em Rasterization} & {\small 73.91} & {\small 75.03} & {\small 74.38} & {\small 75.36} & {\small 75.91} \\
{\small\em Sampling} & {\small 93.63} & {\small 91.40} & {\small 89.84} & {\small 88.39} & {\small 89.63} \\
{\small\em Holes} & {\small 94.13} & {\small 92.81} & {\small 91.68} & {\small 90.79} & {\small 90.16} \\
{\small\em Micro holes} & {\small 93.24} & {\small 92.13} & {\small 90.97} & {\small 90.04} & {\small 89.30} \\
{\small\em Scaling} & {\small 98.85} & {\small 98.85} & {\small 98.85} & {\small 98.85} & {\small 98.85} \\
{\small\em Affine} & {\small 96.51} & {\small 96.66} & {\small 96.91} & {\small 96.76} & {\small 96.49} \\
{\small\em Noise} & {\small 94.53} & {\small 95.05} & {\small 95.23} & {\small 95.37} & {\small 95.43} \\
{\small\em Shot Noise} & {\small 94.29} & {\small 93.72} & {\small 93.57} & {\small 93.47} & {\small 93.47} \\
{\small\em Partial} & {\small 98.65} & {\small 98.23} & {\small 98.20} & {\small 97.61} & {\small 97.86} \\
{\small\em View} & {\small 97.77} & {\small 97.53} & {\small 97.55} & {\small 97.28} & {\small 97.05} \\
\hline
{\small{\textbf{Average}}} & {\small 93.95} & {\small 93.63} & {\small 93.27} & {\small 92.97} & {\small 92.99} \\
\hline
\end{tabular}
\caption{\small Repeatability (in $\%$) at $\rho=5$ of Mesh-Scale DoG (2) feature detection algorithm. Average number of detected points: 1538.\label{tab:keller_spin-1}}
\end{table}

==> results/keller_spin.feat.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 99.75} & {\small 99.83} & {\small 99.85} & {\small 99.87} & {\small 99.87} \\
{\small\em Rasterization} & {\small 98.25} & {\small 98.28} & {\small 98.23} & {\small 98.26} & {\small 98.17} \\
{\small\em Sampling} & {\small 99.62} & {\small 99.61} & {\small 99.52} & {\small 99.40} & {\small 99.52} \\
{\small\em Holes} & {\small 99.75} & {\small 99.76} & {\small 99.70} & {\small 99.67} & {\small 99.61} \\
{\small\em Micro holes} & {\small 99.25} & {\small 99.29} & {\small 99.26} & {\small 99.25} & {\small 99.20} \\
{\small\em Scaling} & {\small 99.92} & {\small 99.92} & {\small 99.92} & {\small 99.92} & {\small 99.92} \\
{\small\em Affine} & {\small 99.73} & {\small 99.83} & {\small 99.83} & {\small 99.83} & {\small 99.83} \\
{\small\em Noise} & {\small 99.94} & {\small 99.92} & {\small 99.92} & {\small 99.92} & {\small 99.91} \\
{\small\em Shot Noise} & {\small 99.74} & {\small 99.75} & {\small 99.74} & {\small 99.71} & {\small 99.71} \\
{\small\em Partial} & {\small 99.91} & {\small 99.88} & {\small 99.90} & {\small 99.82} & {\small 99.85} \\
{\small\em View} & {\small 99.97} & {\small 99.89} & {\small 99.88} & {\small 99.84} & {\small 99.84} \\
\hline
{\small{\textbf{Average}}} & {\small 99.62} & {\small 99.63} & {\small 99.61} & {\small 99.59} & {\small 99.58} \\
\hline
\end{tabular}
\caption{\small Repeatability (in $\%$) at $\rho=5$ of Mesh-Scale DoG (1) feature detection algorithm. Average number of detected points: 3616.\label{tab:keller_spin}}
\end{table}

==> results/l2norm/Zaharescu_corr-det1-feat1-pt400.desc.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 0.17} & {\small 0.17} & {\small 0.19} & {\small 0.19} & {\small 0.21} \\
{\small\em Rasterization} & {\small 1.00} & {\small 1.00} & {\small 0.99} & {\small 0.99} & {\small 0.99} \\
{\small\em Sampling} & {\small 0.93} & {\small 0.95} & {\small 0.96} & {\small 0.97} & {\small 0.98} \\
{\small\em Holes} & {\small 0.23} & {\small 0.24} & {\small 0.26} & {\small 0.29} & {\small 0.32} \\
{\small\em Micro holes} & {\small 0.30} & {\small 0.31} & {\small 0.33} & {\small 0.34} & {\small 0.35} \\
{\small\em Scaling} & {\small 0.20} & {\small 0.20} & {\small 0.20} & {\small 0.20} & {\small 0.20} \\
{\small\em Affine} & {\small 0.52} & {\small 0.63} & {\small 0.68} & {\small 0.72} & {\small 0.75} \\
{\small\em Noise} & {\small 1.00} & {\small 0.99} & {\small 0.99} & {\small 0.99} & {\small 0.99} \\
{\small\em Shot Noise} & {\small 0.23} & {\small 0.24} & {\small 0.25} & {\small 0.26} & {\small 0.27} \\
{\small\em Partial} & {\small 0.30} & {\small 0.36} & {\small 0.37} & {\small 0.46} & {\small 0.49} \\
{\small\em View} & {\small 0.64} & {\small 0.59} & {\small 0.61} & {\small 0.60} & {\small 0.60} \\
\hline
{\small{\textbf{Average}}} & {\small 0.50} & {\small 0.52} & {\small 0.53} & {\small 0.55} & {\small 0.56} \\
\hline
\end{tabular}
\caption{\small Quality of Mesh HoG feature description algorithm (average normalized $L_2$ distance between descriptors at corresponding points) on feature points detected using Mesh DoG (mean). Average number of points: 392.\label{tab:Zaharescu_corr-det1-feat1-pt400}}
\end{table}

==> results/l2norm/Zaharescu_corr-det2-feat2-pt400.desc.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 0.15} & {\small 0.15} & {\small 0.17} & {\small 0.17} & {\small 0.19} \\
{\small\em Rasterization} & {\small 0.98} & {\small 0.98} & {\small 0.99} & {\small 0.99} & {\small 0.99} \\
{\small\em Sampling} & {\small 0.95} & {\small 0.97} & {\small 0.97} & {\small 0.98} & {\small 0.98} \\
{\small\em Holes} & {\small 0.21} & {\small 0.23} & {\small 0.27} & {\small 0.30} & {\small 0.34} \\
{\small\em Micro holes} & {\small 0.29} & {\small 0.30} & {\small 0.32} & {\small 0.34} & {\small 0.35} \\
{\small\em Scaling} & {\small 0.19} & {\small 0.19} & {\small 0.19} & {\small 0.19} & {\small 0.19} \\
{\small\em Affine} & {\small 0.58} & {\small 0.66} & {\small 0.71} & {\small 0.74} & {\small 0.78} \\
{\small\em Noise} & {\small 0.98} & {\small 0.99} & {\small 0.99} & {\small 0.99} & {\small 0.99} \\
{\small\em Shot Noise} & {\small 0.22} & {\small 0.23} & {\small 0.24} & {\small 0.25} & {\small 0.26} \\
{\small\em Partial} & {\small 0.32} & {\small 0.40} & {\small 0.40} & {\small 0.48} & {\small 0.51} \\
{\small\em View} & {\small 0.69} & {\small 0.62} & {\small 0.65} & {\small 0.65} & {\small 0.63} \\
\hline
{\small{\textbf{Average}}} & {\small 0.51} & {\small 0.52} & {\small 0.54} & {\small 0.55} & {\small 0.56} \\
\hline
\end{tabular}
\caption{\small Quality of Mesh HoG feature description algorithm (average normalized $L_2$ distance between descriptors at corresponding points) on feature points detected using Mesh DoG (Gaussian). Average number of points: 391.\label{tab:Zaharescu_corr-det2-feat2-pt400}}
\end{table}

==> results/l2norm/Zobel_Valentin_GHKS.desc.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 0.99} & {\small 1.01} & {\small 1.01} & {\small 1.01} & {\small 1.01} \\
{\small\em Rasterization} & {\small --} & {\small --} & {\small --} & {\small --} & {\small --} \\
{\small\em Sampling} & {\small 1.01} & {\small 1.01} & {\small 1.01} & {\small 1.01} & {\small 1.01} \\
{\small\em Holes} & {\small --} & {\small --} & {\small --} & {\small --} & {\small --} \\
{\small\em Micro holes} & {\small --} & {\small --} & {\small --} & {\small --} & {\small --} \\
{\small\em Scaling} & {\small 1.01} & {\small 1.02} & {\small 1.02} & {\small 1.01} & {\small 1.01} \\
{\small\em Affine} & {\small 1.02} & {\small 1.04} & {\small 1.04} & {\small 1.03} & {\small 1.03} \\
{\small\em Noise} & {\small 1.02} & {\small 1.02} & {\small 1.03} & {\small 1.02} & {\small 1.02} \\
{\small\em Shot Noise} & {\small 1.04} & {\small 1.01} & {\small 1.00} & {\small 1.01} & {\small 1.02} \\
{\small\em Partial} & {\small 0.99} & {\small 1.00} & {\small 1.01} & {\small 1.00} & {\small 1.00} \\
{\small\em View} & {\small --} & {\small --} & {\small --} & {\small --} & {\small --} \\
%\hline
%{\small{\textbf{Average}}} & {\small 0.28} & {\small 0.28} & {\small 0.28} & {\small 0.28} & {\small 0.28} \\
\hline
\end{tabular}
\caption{\small Quality of GHKS feature description algorithm (average normalized $L_2$ distance between descriptors at corresponding points).\label{tab:Zobel_Valentin_GHKS}}
\end{table}

==> results/l2norm/keller_sift-1.desc.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 0.67} & {\small 0.61} & {\small 0.64} & {\small 0.65} & {\small 0.64} \\
{\small\em Rasterization} & {\small 0.95} & {\small 0.96} & {\small 0.96} & {\small 0.96} & {\small 0.96} \\
{\small\em Sampling} & {\small 0.79} & {\small 0.81} & {\small 0.85} & {\small 0.87} & {\small 0.90} \\
{\small\em Holes} & {\small 0.79} & {\small 0.82} & {\small 0.84} & {\small 0.86} & {\small 0.87} \\
{\small\em Micro holes} & {\small 0.78} & {\small 0.80} & {\small 0.83} & {\small 0.84} & {\small 0.86} \\
{\small\em Scaling} & {\small 0.71} & {\small 0.72} & {\small 0.74} & {\small 0.75} & {\small 0.76} \\
{\small\em Affine} & {\small 0.89} & {\small 0.89} & {\small 0.91} & {\small 0.92} & {\small 0.94} \\
{\small\em Noise} & {\small 0.95} & {\small 0.96} & {\small 0.97} & {\small 0.98} & {\small 0.98} \\
{\small\em Shot Noise} & {\small 0.79} & {\small 0.81} & {\small 0.82} & {\small 0.83} & {\small 0.84} \\
{\small\em Partial} & {\small 0.50} & {\small 0.51} & {\small 0.57} & {\small 0.61} & {\small 0.63} \\
{\small\em View} & {\small 0.84} & {\small 0.82} & {\small 0.83} & {\small 0.83} & {\small 0.83} \\
\hline
{\small{\textbf{Average}}} & {\small 0.79} & {\small 0.79} & {\small 0.81} & {\small 0.83} & {\small 0.84} \\
\hline
\end{tabular}
\caption{\small Quality of Local depth SIFT feature description algorithm (average normalized $L_2$ distance between descriptors at corresponding points) on feature points detected using Interest point (1). Average number of points: 1538.\label{tab:keller_sift-1}}
\end{table}

==> results/l2norm/keller_sift.desc.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 0.63} & {\small 0.56} & {\small 0.58} & {\small 0.59} & {\small 0.59} \\
{\small\em Rasterization} & {\small 0.94} & {\small 0.94} & {\small 0.94} & {\small 0.94} & {\small 0.94} \\
{\small\em Sampling} & {\small 0.74} & {\small 0.77} & {\small 0.81} & {\small 0.84} & {\small 0.87} \\
{\small\em Holes} & {\small 0.71} & {\small 0.73} & {\small 0.75} & {\small 0.77} & {\small 0.78} \\
{\small\em Micro holes} & {\small 0.70} & {\small 0.74} & {\small 0.76} & {\small 0.78} & {\small 0.80} \\
{\small\em Scaling} & {\small 0.68} & {\small 0.70} & {\small 0.72} & {\small 0.74} & {\small 0.75} \\
{\small\em Affine} & {\small 0.87} & {\small 0.88} & {\small 0.90} & {\small 0.91} & {\small 0.93} \\
{\small\em Noise} & {\small 0.95} & {\small 0.96} & {\small 0.97} & {\small 0.98} & {\small 0.98} \\
{\small\em Shot Noise} & {\small 0.70} & {\small 0.73} & {\small 0.76} & {\small 0.78} & {\small 0.80} \\
{\small\em Partial} & {\small 0.46} & {\small 0.47} & {\small 0.53} & {\small 0.57} & {\small 0.59} \\
{\small\em View} & {\small 0.76} & {\small 0.74} & {\small 0.75} & {\small 0.74} & {\small 0.74} \\
\hline
{\small{\textbf{Average}}} & {\small 0.74} & {\small 0.75} & {\small 0.77} & {\small 0.79} & {\small 0.80} \\
\hline
\end{tabular}
\caption{\small Quality of Local depth SIFT feature description algorithm (average normalized $L_2$ distance between descriptors at corresponding points) on feature points detected using Interest point (1). Average number of points: 3616.\label{tab:keller_sift}}
\end{table}

==> results/l2norm/keller_spin-1.desc.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 0.29} & {\small 0.55} & {\small 0.64} & {\small 0.55} & {\small 0.60} \\
{\small\em Rasterization} & {\small 0.91} & {\small 0.90} & {\small 0.89} & {\small 0.89} & {\small 0.90} \\
{\small\em Sampling} & {\small 0.67} & {\small 0.71} & {\small 0.74} & {\small 0.78} & {\small 0.82} \\
{\small\em Holes} & {\small 0.50} & {\small 0.55} & {\small 0.59} & {\small 0.62} & {\small 0.65} \\
{\small\em Micro holes} & {\small 0.89} & {\small 0.90} & {\small 0.90} & {\small 0.91} & {\small 0.92} \\
{\small\em Scaling} & {\small 0.26} & {\small 0.26} & {\small 0.26} & {\small 0.26} & {\small 0.26} \\
{\small\em Affine} & {\small 0.64} & {\small 0.77} & {\small 0.77} & {\small 0.78} & {\small 0.81} \\
{\small\em Noise} & {\small 0.93} & {\small 0.95} & {\small 0.96} & {\small 0.96} & {\small 0.97} \\
{\small\em Shot Noise} & {\small 0.51} & {\small 0.55} & {\small 0.58} & {\small 0.60} & {\small 0.62} \\
{\small\em Partial} & {\small 0.80} & {\small 0.80} & {\small 0.80} & {\small 0.72} & {\small 0.66} \\
{\small\em View} & {\small 0.63} & {\small 0.58} & {\small 0.60} & {\small 0.59} & {\small 0.59} \\
\hline
{\small{\textbf{Average}}} & {\small 0.64} & {\small 0.68} & {\small 0.70} & {\small 0.70} & {\small 0.71} \\
\hline
\end{tabular}
\caption{\small Quality of Scale invariant Spin Image feature description algorithm (average normalized $L_2$ distance between descriptors at corresponding points) on feature points detected using Interest point (1). Average number of points: 1538.\label{tab:keller_spin-1}}
\end{table}

==> results/l2norm/keller_spin.desc.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 0.26} & {\small 0.52} & {\small 0.61} & {\small 0.52} & {\small 0.57} \\
{\small\em Rasterization} & {\small 0.88} & {\small 0.87} & {\small 0.87} & {\small 0.87} & {\small 0.87} \\
{\small\em Sampling} & {\small 0.62} & {\small 0.66} & {\small 0.70} & {\small 0.75} & {\small 0.79} \\
{\small\em Holes} & {\small 0.36} & {\small 0.39} & {\small 0.42} & {\small 0.45} & {\small 0.47} \\
{\small\em Micro holes} & {\small 0.84} & {\small 0.85} & {\small 0.86} & {\small 0.87} & {\small 0.87} \\
{\small\em Scaling} & {\small 0.24} & {\small 0.24} & {\small 0.24} & {\small 0.24} & {\small 0.24} \\
{\small\em Affine} & {\small 0.60} & {\small 0.74} & {\small 0.75} & {\small 0.76} & {\small 0.79} \\
{\small\em Noise} & {\small 0.96} & {\small 0.97} & {\small 0.98} & {\small 0.98} & {\small 0.99} \\
{\small\em Shot Noise} & {\small 0.41} & {\small 0.48} & {\small 0.52} & {\small 0.56} & {\small 0.60} \\
{\small\em Partial} & {\small 0.78} & {\small 0.77} & {\small 0.78} & {\small 0.69} & {\small 0.62} \\
{\small\em View} & {\small 0.50} & {\small 0.45} & {\small 0.46} & {\small 0.46} & {\small 0.45} \\
\hline
{\small{\textbf{Average}}} & {\small 0.58} & {\small 0.63} & {\small 0.65} & {\small 0.65} & {\small 0.66} \\
\hline
\end{tabular}
\caption{\small Quality of Scale invariant Spin Image feature description algorithm (average normalized $L_2$ distance between descriptors at corresponding points) on feature points detected using Interest point (0). Average number of points: 3616.\label{tab:keller_spin}}
\end{table}

==> results/vw_table_matchingScore.tex <==
\begin{table}
\centering
\begin{tabular}{lccccc}
& \multicolumn{5}{c}{\small\textbf{ Strength}} \\
\cline{2-6}
{\small\textbf{ Transform.}} & {\small\textbf{  1}} & {\small\textbf{ $\leq$2}} & {\small\textbf{ $\leq$3}} & {\small\textbf{ $\leq$4}} & {\small\textbf{ $\leq$5}}\\
\hline
{\small\em Isometry} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 100.00}\\
{\small\em Rasterization} & {\small 66.67} & {\small 72.22} & {\small 59.26} & {\small 44.44} & {\small 35.56}\\
{\small\em Sampling} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 75.00} & {\small 60.00}\\
{\small\em Holes} & {\small 100.00} & {\small 50.00} & {\small 33.33} & {\small 25.00} & {\small 21.76}\\
{\small\em Micro holes} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 96.88} & {\small 86.39}\\
{\small\em Scaling} & {\small 100.00} & {\small 100.00} & {\small 100.00} & {\small 84.38} & {\small 85.00}\\
{\small\em Affine} & {\small 75.00} & {\small 56.25} & {\small 46.59} & {\small 39.94} & {\small 41.95}\\
{\small\em Noise} & {\small 100.00} & {\small 100.00} & {\small 91.67} & {\small 79.86} & {\small 71.89}\\
{\small\em Shot Noise} & {\small 100.00} & {\small 94.44} & {\small 81.48} & {\small 75.00} & {\small 68.89}\\
{\small\em Partial} & {\small 75.00} & {\small 68.75} & {\small 60.12} & {\small 51.34} & {\small 41.07}\\
{\small\em View} & {\small 0.00} & {\small 50.00} & {\small 51.52} & {\small 51.14} & {\small 42.73}\\
\hline
{\small{\textbf{Average}}} & {\small 83.33} & {\small 81.06} & {\small 74.91} & {\small 65.72} & {\small 59.57}\\
\hline
\end{tabular}
\caption{\small Robustness of SI-HKS region description algorithm ($\%$ of nearest neighbors with overlap {\em overlap $\geq$ 70\%}) on stable regions detected using vertex-weight $h_t(v,v)$ .\label{}}
\end{table}
